Learning sources of variability from high-dimensional observational studies

Causal inference studies whether the presence of a variable influences an observed outcome. As measured by quantities such as the "average treatment effect," this paradigm is employed across numerous biological fields, from vaccine and drug development to policy interventions. Unfortunately, the majority of these methods are often limited to univariate outcomes. Our work generalizes causal estimands to outcomes with any number of dimensions or any measurable space, and formulates traditional causal estimands for nominal variables as causal discrepancy tests. We propose a simple technique for adjusting universally consistent conditional independence tests and prove that these tests are universally consistent causal discrepancy tests. Numerical experiments illustrate that our method, Causal CDcorr, leads to improvements in both finite sample validity and power when compared to existing strategies. Our methods are all open source and available at github.com/ebridge2/cdcorr.

==> Content/background.tex <==

\section{Background}

The average treatment effect \cite{Rubin1974,Athey2017May} forms the backbone of many investigations in causal inference. We obtain the observed data $(y_i, t_i,  x_i)$, where $y_i \in \mathbb R$ is the outcome, $t_i \in \{1, 2\}$ is the (binary) treatment/intervention of interest (either treated or untreated), and $ x_i$ are the vector of baseline covariates (potential confounders), for individuals $i \in [n]$. To investigate this problem, we assume the existence of three random variables, $(\mathbf y_i, \mathbf t_i, {\mathbf x}_i)$, which are sampled independently and identically from some unknown data-generating distribution $F_{\mathbf y_i, \mathbf t_i, \mathbf x_i}$. Additionally, we assume the existence of two counterfactual random variables, $\mathbf y_i(1)$ and $\mathbf y_i(2)$, which represent the \textit{potential} outcomes under the two possible treatments. Conceptually, the theory of causal inference rests on the \textbf{consistency} assumption, which asserts that there is a single \textit{version} of each treatment level; e.g., if $\mathbf t_i = t$, then $\mathbf y_i = \mathbf y_i(t)$ \cite{Cole2009Jan}. Under this framework, the observed outcome is:
\begin{align*}
    \mathbf y_i &= \mathbf y_i(1) \indicator{\mathbf t_i = 1} + \mathbf y_i(2) \indicator{\mathbf t_i = 2},
\end{align*}
where only one of the potential outcomes will actually be realized in the observed data. The average treatment effect ($ATE$) is given by:
\begin{align}
    \gamma \triangleq ATE = \expect{\mathbf y_i(2) - \mathbf y_i(1)} = \expect{\mathbf y_i(2)} - \expect{\mathbf y_i(1)}
\end{align}
To test whether there is an $ATE$ implies the following hypothesis test:
\begin{align}
    H_0 : \gamma = 0 \text{ against }H_A: \gamma \neq 0.
\end{align}

The most obvious issue regarding the ATE is that, in practice, we observe realizations of $\mathbf y_i$ (the observed data), and \textit{not} $\mathbf y_i(t)$ (the counterfactual data); this is known as the ``fundamental problem of causal inference.'' When is $\expect{\mathbf y_i(t)}$ identifiable from the observed data, and how do we identify it?

The identifiability of $\expect{\mathbf y_i(t)}$ is ensured by the \textit{ignorability}, \textit{consistency}, \textit{positivity}, and the \textit{no interference} constraints. \textbf{Ignorability} is said to hold provided that $(\mathbf y_i(2), \mathbf y_i(1)) \indep \mathbf t_i \cond {\mathbf x}_i$; that is, the treatment is independent with respect to the observed baseline covariates. This condition will hold if the study executes it by design (such as in a perfect randomized trial) or all confounders have been recorded with the baseline covariates \cite{Holland1986}. The \textit{consistency} assumption is described above. \textbf{Positivity} holds if, for each possible treatment $t$, $Pr(\mathbf t_i = t \cond  {\mathbf x}_i =  x) > 0$ for any $ x$ in the support of ${\mathbf x}_i$ \cite{Rosenbaum1985,Rosenbaum2010}. Conceptually, any possible individual with a given covariate level \textit{could} have been observed in either the treated or untreated group. \textbf{No interference} asserts that there is no impact between the treatment assignments of \textit{other} participants on the potential outcomes of a given participant; this allows $\mathbf y_i(k)$ to be well-defined without reference to other individuals' treatment assignments \cite{Hernán2006}. When the consistency and no interference assumptions hold, these two assumptions are collectively referred to as the \textbf{Stable-Unit Treatment Value Assumption} (SUTVA) \cite{Hernán2006,Imbens2015,Rubin1980}. 

Under the $G$-computation formula \cite{Robins1986Jan}, if these assumptions hold, then:
\begin{align*}
    \expect{\mathbf y_i(t)} &= \expect{\expect{\mathbf y_i \cond \mathbf t_i = t,  {\mathbf x}_i}},
\end{align*}
and the ATE can be expressed as
\begin{align}
    \gamma &= \expect{\expect{\mathbf y_i \cond \mathbf t_i = 2,  {\mathbf x}_i}} - \expect{ \expect{\mathbf y_i \cond \mathbf t_i = 1, {\mathbf x}_i}}.
    \label{eqn:g_comp}
\end{align}
% Su/White? Weighted hellinger distance stuff? conditional ch.f. stuff? max nlin conditional corr?
As a general measure of treatment effects, the average treatment effect, as defined above, is rather limiting. First, treatment effects aren't necessarily constant across all individuals. One could conceptualize an intervention which has a strongly positive effect on younger people, but has a negative effect on older people. The average treatment effect ends up "averaging away" the heterogeneous effect of treatment on younger and older people, with the average treatment effect ending up being zero. This has been overcome by study of conditional (on baseline covariates, such as age) average treatment effects (the $CATE$) \cite{hahn1998role}: 
\begin{align*}
    \gamma_x \triangleq CATE(x) = \expect{\mathbf y_i(2) - \mathbf y_i(1) \cond \mathbf x_i = x} = \expect{\mathbf y_i(2) \cond \mathbf x_i = x} - \expect{\mathbf y_i(1) \cond \mathbf x_i = x}
\end{align*}
and a relevant test is whether, for each possible $x$:
\begin{align}
    H_0 : \gamma_x = 0 \text{ against }H_A: \gamma_x \neq 0,
    \label{eqn:hypo_cate}
\end{align}
but these too are not without limitations. 


==> Content/extra_stuff.tex <==

\begin{comment}
\begin{lemma}[Equivalent characterization for density of a potential outcome]
Assume the setup described in \ref{setup}. Further, suppose that:
\begin{enumerate}
    \item The treatment assignment is ignorable: $\parens*{\mathbf y_i(1), ..., \mathbf y_i(K)} \indep \mathbf t_i \cond \mathbf x_i$,
    \item The treatment assignments are positive for all levels of the covariates: $\prob{\mathbf t_i = k \cond \mathbf x_i = x} > 0$ for any $x \in \mathcal X$, and
    \item No interference: if $i \neq j$, then $\mathbf y_i(k) \indep \mathbf t_j$ for all $k \in [K]$.
\end{enumerate}
Then:
\begin{align*}
    f_{\mathbf y_i(k)}(y) &= \int_{\mathcal X}f_{\mathbf y_i | \mathbf t_i = k, x}(y) f_{\mathbf x_i}(x) \,\text d x.
\end{align*}
\label{lem:equiv_char}
\end{lemma}
\begin{proof}
By definition, $f_{\mathbf y_i(k)}(y)$ can be expressed as a marginalization over the joint density $f_{\mathbf y_i(k), \mathbf x_i, \mathbf t_i}(y,t,x)$ with respect to $\mathbf x_i$ and $\mathbf t_i$:
\begin{align*}
    f_{\mathbf y_i(k)}(y) &= \int_{\mathcal X \times \mathcal T}
    f_{\mathbf y_i(k) | t, x}(y)f_{\mathbf x_i, \mathbf t_i}(x, t)\,\text d (x,t),
\end{align*}

Using the definition of conditional probability gives:
\begin{align*}
    f_{\mathbf y_i(k)}(y) &= \int_{\mathcal X \times \mathcal T}
    f_{\mathbf y_i(k) | t, x}(y)\prob{\mathbf t_i = t | \mathbf x_i = x}f_{\mathbf x_i}(x)\,\text d (x,t).
\end{align*}
That the treatment levels are positive for all levels of the covariates gives that this quantity is well-defined. By Fubini's theorem, and using that $\mathcal T = [K]$ is discrete:
\begin{align*}
    f_{\mathbf y_i(k)}(y) &= \int_{\mathcal X}\bracks*{\sum_{t \in [K]}\parens*{
    f_{\mathbf y_i(k) | t, x}(y) - f_{\mathbf y_i(l) | t, x}(y)}\prob{\mathbf t_i = t | \mathbf x_i = x}} f_{\mathbf x_i}(x)\,\text d x.
\end{align*}

By ignorability, $f_{\mathbf y_i(k) | t, x}(y) = f_{\mathbf y_i(k) | k, x}(y)$, so:
\begin{align*}
    f_{\mathbf y_i(k)}(y) - f_{\mathbf y_i(l)}(y) &= \int_{\mathcal X}\bracks*{\sum_{t \in [K]}
    f_{\mathbf y_i(k) | k, x}(y)\prob{\mathbf t_i = t | \mathbf x_i = x}} f_{\mathbf x_i}(x)\,\text d x.
\end{align*}
By consistency:
\begin{align*}
    f_{\mathbf y_i(k)}(y) &= \int_{\mathcal X}\bracks*{\sum_{t \in [K]}
    f_{\mathbf y_i | k, x}(y)\prob{\mathbf t_i = t | \mathbf x_i = x}} f_{\mathbf x_i}(x)\,\text d x.
\end{align*}
Finally, since $f_{\mathbf y_i | k, x}(y)$ is constant with respect to $t$:
\begin{align*}
    f_{\mathbf y_i(k)}(y) &= \int_{\mathcal X}
    f_{\mathbf y_i | k, x}(y)\bracks*{\sum_{t \in [K]}\prob{\mathbf t_i = t | \mathbf x_i = x}} f_{\mathbf x_i}(x)\,\text d x \\
    &= \int_{\mathcal X}
    f_{\mathbf y_i | k, x}(y) f_{\mathbf x_i}(x)\,\text d x, \,\,\,\, \sum_{t \in [K]}\prob{\mathbf t_i = t | \mathbf x_i = x} = 1.
\end{align*}
\end{proof}
\end{comment}


\begin{comment}
\paragraph{Causal treatment effects on the treated}
A related causal estimand which is commonly estimated in practice is the \textit{conditional average treatment effect on the treated} (CATT). This estimand is practically related to the CATE in \ref{eqn:hypo_cate}, but with a few subtle differences:
\begin{align*}
    \tau_x &\triangleq \expect{\mathbf y_i(2) \cond \mathbf x_i = x, \mathbf t_i = 2} - \expect{\mathbf y_i(1) \cond  \mathbf x_i = x, \mathbf t_i = 2}.
\end{align*}
The idea here is that, whereas $\gamma_x$ represents the realized difference in expectation of an item $i$'s counterfactuals conditional on having baseline covariates $x$, $\tau_x$ makes the more generic step of conditioning to take the difference in expectation of an item $i$'s counterfactuals \textit{only for the treated group}. The subtle difference is that with $\tau_x$, we make no statements about the entire population under consideration: we make only statements about the treated population. 

Since this concept is less restrictive than $\gamma_x$, intuitively, fewer requirements have to be met in order to estimate $\tau_x$ identifiably from the data. In particular, to estimate $\tau_x$, the only criteria we need are \textit{ignorability}, \textit{consistency} and \textit{exact matching}. While we already learned about consistency and ignorability, \textbf{exact matching} means that $F_{\mathbf x_i | \mathbf t_i = 2} = F_{\mathbf x_i | \mathbf t_i = 1}$: the distribution of the covariates are the same in the treatment and control groups. This has a key implication for condition 4 under Setup \ref{setup}: the covariates conditional on the treatments have positive support. For any $x \in \mathcal X$:
\begin{align*}
    f_{\mathbf x_i}(x) &= \sum_{t \in [2]}f_{\mathbf x_i | \mathbf t_i = t}(x)\prob{\mathbf t_i = t} \\
    &= f_{\mathbf x_i | \mathbf t_i = t'}(x)\sum_{t \in [2]}\prob{\mathbf t_i = t},\,\,\,\,F_{\mathbf x_i | \mathbf t_i = 1} = F_{\mathbf x_i | \mathbf t_i = 2} \\
    &= f_{\mathbf x_i | \mathbf t_i = t'}(x).\,\,\,\,\sum_{t \in [2]}\prob{\mathbf t_i = t} = 1\numberthis \label{eqn:cond4_CDTT}
\end{align*}
which holds for any $t' \in [2]$. This fact will be useful for hypothesis testing, in Section \ref{sec:methods}, for delineating that we are testing well-defined quantities.

To generalize the concept of an average treatment effect on the treated, we define the estimand:

\begin{definition}[Distributional treatment effect on the treated]
Suppose the setup described in \ref{setup} for the two-group setting, where group $2$ is defined as the treatment group, and group $1$ is defined as the control group. A causal categorical treatment effect on the treated (\textbf{DTT}) exists if for some $x \in \mathcal X$:
\begin{align*}
    F_{\mathbf y_i(2) | \mathbf t_i = 2} &\neq F_{\mathbf y_i(1) | \mathbf t_i = 2}
\end{align*}
\label{defn:DTT}
\end{definition}

The nuance here that differentiates this concept from the CoDiCE in Definition \ref{def:CDTE} for the case of $K=2$ is that the distributions of interest here are \textit{conditional} on the treatment group, and \textit{unconditional} on the covariates. This has the intuitive implication that, unlike the CoDiCE, inference here is limited to a population which is distributed like the treatment group, rather than like the entire population under investigation. However, we have strengthened the detected effect to be \textit{global} across levels of the covariates. A suitable hypothesis for a DTT is:

\begin{align}
    H_0 : F_{\mathbf y_i(2) | 2, x} = F_{\mathbf y_i(1) | 2, x}\text{    against     }H_A : F_{\mathbf y_i(2) | \mathbf t_i = 2} \neq F_{\mathbf y_i(1) | \mathbf t_i = 2}
    \label{eqn:hypo_causal_tt}
\end{align}

As before, with some general assumptions, we can express the densities of these potential outcomes in terms of the conditional densities:
\begin{lemma}
Suppose the setup describe in \ref{setup}, where group $2$ is defined as the treatment group, and group $1$ is defined as the control group. Further, suppose that:
\begin{enumerate}
    \item The treatment assignment is ignorable: $\parens*{\mathbf y_i(1), \mathbf y_i(2)} \indep \mathbf t_i \cond \mathbf x_i$,
    \item The covariates are exactly matched: $F_{\mathbf x_i | \mathbf t_i = 2} = F_{\mathbf x_i | \mathbf t_i = 1}$, and
    \item No interference: if $i \neq j$, then $\mathbf y_i(k) \indep \mathbf t_j$ for $k \in [2]$.
\end{enumerate}
Then:
\begin{enumerate}
    \item $$f_{\mathbf y_i(2) | \mathbf t_i = 2}(y) = \int_{\mathcal X}f_{\mathbf y_i | 2, x}(y)f_{\mathbf x_i}(x)\,\text d x,\text{ and}$$
    \item $$f_{\mathbf y_i(1) | \mathbf t_i = 2}(y) = \int_{\mathcal X}f_{\mathbf y_i | 1, x}f_{\mathbf x_i}(x)\,\text d x.$$
\end{enumerate}
\label{lem:CDTT_helper}
\end{lemma}
\begin{proof}
\, \\
1. Note that $f_{\mathbf y_i(2) | \mathbf t_i = 2}(y)$ can be expressed as a marginalization of $f_{\mathbf y_i(2), \mathbf x_i | \mathbf t_i = 2}(y)$ over $\mathbf x_i$. So:
\begin{align*}
f_{\mathbf y_i(2) | \mathbf t_i = 2}(y) &= \int_{\mathcal X}f_{\mathbf y_i(2) | 2, x}(y)f_{\mathbf x_i | \mathbf t_i = 2}(x) \,\text d x.
\end{align*}
Using that consistency gives that $f_{\mathbf y_i(2)|2, x}(y) = f_{\mathbf y_i | 2, x}(y)$ and Equation \ref{eqn:cond4_CDTT} gives:
\begin{align*}
f_{\mathbf y_i(2) | \mathbf t_i = 2}(y) &= \int_{\mathcal X}f_{\mathbf y_i | 2, x}(y)f_{\mathbf x_i | \mathbf t_i = 2}(x) \,\text d x.
\end{align*}
2. Note that $f_{\mathbf y_i(1) | \mathbf t_i = 2}(y)$ can be expressed as a marginalization of $f_{\mathbf y_i(2), \mathbf x_i | \mathbf t_i = 2}(y)$ over $\mathbf x_i$:
\begin{align*}
f_{\mathbf y_i(1) | 2, x}(y) &= \int_{\mathcal X}f_{\mathbf y_i(1) | 2, x}(y)f_{\mathbf x_i | \mathbf t_i = 2}(x)\,\text d x.
\end{align*}
By ignorability, $f_{\mathbf y_i(1) | 2, x}(y) = f_{\mathbf y_i(1) | 1, x}(y)$, so:
\begin{align*}
f_{\mathbf y_i(1) | 2, x}(y) &= \int_{\mathcal X}f_{\mathbf y_i(1) | 1, x}(y)f_{\mathbf x_i | \mathbf t_i = 2}(x)\,\text d x.
\end{align*}
Using consistency, $f_{\mathbf y_i(1) | 1, x}(y) = f_{\mathbf y_i | 1, x}(y)$:
\begin{align*}
f_{\mathbf y_i(1) | 2, x}(y) &= \int_{\mathcal X}f_{\mathbf y_i | 1, x}(y)f_{\mathbf x_i | \mathbf t_i = 2}(x)\,\text d x \\
&= \int_{\mathcal X}f_{\mathbf y_i | 1, x}(y)f_{\mathbf x_i}(x)\,\text d x.\,\,\,\,\text{Equation \ref{eqn:cond4_CDTT}}
\end{align*}
\end{proof}

Under assumptions given in Lemma \ref{lem:CDTT_helper}, a test of Equation \eqref{eqn:hypo_cond_kst} is a test of a CDTT:
\begin{theorem}[$k$-sample testing and CDTT]
Suppose the setup describe in \ref{setup}, where group $2$ is defined as the treatment group, and group $1$ is defined as the control group. Further, suppose that:
\begin{enumerate}
    \item The treatment assignment is ignorable: $\parens*{\mathbf y_i(1), \mathbf y_i(2)} \indep \mathbf t_i \cond \mathbf x_i$,
    \item The covariates are exactly matched: $F_{\mathbf x_i | \mathbf t_i = 2} = F_{\mathbf x_i | \mathbf t_i = 1}$, and
    \item No interference: if $i \neq j$, then $\mathbf y_i(k) \indep \mathbf t_j$ for $k \in [2]$.
\end{enumerate}
Then a consistent test of Equation \eqref{eqn:hypo_cond_kst} is equivalent to a consistent test of \eqref{eqn:hypo_causal_tt} for a CDTT.
\label{thm:CDTT}
\end{theorem}

\begin{proof}
Recall that for Equations \ref{eqn:hypo_cond_kst} and \ref{eqn:hypo_causal_tt} that since the density fully determines a distribution, that a difference in distribution exists $\iff$ a difference in the densities exists.

By Lemma \ref{lem:CDTT_helper}, Equation \ref{eqn:hypo_causal_tt} can be expressed in terms of the relevant densities from Equation \ref{eqn:hypo_cond_kst}:
\begin{align*}
    f_{\mathbf y_i(k) | \mathbf t_i = 2}(y) - f_{\mathbf y_i(l) \mathbf t_i = 2}(y) &= \int_{\mathcal X}\parens*{f_{\mathbf y_i | k, x}(y) - f_{\mathbf y_i | l, x}(y)} f_{\mathbf x_i}(x) \,\text d x.
\end{align*}
By supposition 4 in Setup \ref{setup}, $f_{\mathbf x_i}(x) > 0$ for all $x \in \mathcal X$. Therefore, $f_{\mathbf y_i(k) | \mathbf t_i = 2}(y) \neq f_{\mathbf y_i(l) \mathbf t_i = 2}(y)$ if and only if there exists some $x \in \mathcal X$ s.t. $f_{\mathbf y_i | k, x}(y) \neq f_{\mathbf y_i | l, x}(y)$, as desired.
\end{proof}
The subtle difference between Theorems \ref{thm:CDTT} and \ref{thm:CDTE} is that we have replaced the \textit{positivity} condition in \ref{thm:CDTE} with the \textit{exact matching} condition in \ref{thm:CDTT}. In theory, the positivity condition might sound easier to achieve: all that we need to know is that there is a non-zero probability of an element being in a particular group given a baseline covariate. On the other hand, with exact matching, we need to \textit{know} that the covariate distributions are equal in each group. In practice, however, the implications of this are substantial. Without a fully randomized design, it is difficult to determine whether the positivity condition holds. However, we can take steps to ensure that the exact matching criterion \textit{approximately} holds. To do this, we leverage re-weighting approaches. Through re-weighting, we upweight (or downweight) individuals in the control group until the covariate distributions are conditionally approximately equivalent between the control and the treatment groups. In this sense, this estimand prioritizes \textit{internal validity} of inference, or the degree to which inference learned from the study sample (which, distributional, is \textit{aligned} to the treatment group) applies to the population of interest (which, in this case, is a population which has a distribution similar to the treatment group.
\end{comment}

% Kernel conditional discrepency test
% CoDiTE

==> preamble.tex <==
%===============================================================================%
% This is the project specific preamble for the ND-latex-template.
%
% If you need a specific package please load it here.
% You can either put an `\input{preamble.tex}` before or after the
% `\usepackage{neurodata}` and deal with any clashes yourself.
% It is important to know which packages clash with our base
% requirements. Thank you
%===============================================================================%


\usepackage{lipsum}
\usepackage{math}
